Stable Real-Time Feedback Control of a Pneumatic Soft Robot

Soft actuators offer compliant and safe interaction with an unstructured environment compared to their rigid counterparts. However, control of these systems is often challenging because they are inherently under-actuated, have infinite degrees of freedom (DoF), and their mechanical properties can change by unknown external loads. Existing works mainly relied on discretization and reduction, suffering from either low accuracy or high computational cost for real-time control purposes. Recently, we presented an infinite-dimensional feedback controller for soft manipulators modeled by partial differential equations (PDEs) based on the Cosserat rod theory. In this study, we examine how to implement this controller in real-time using only a limited number of actuators. To do so, we formulate a convex quadratic programming problem that tunes the feedback gains of the controller in real time such that it becomes realizable by the actuators. We evaluated the controller's performance through experiments on a physical soft robot capable of planar motions and show that the actual controller implemented by the finite-dimensional actuators still preserves the stabilizing property of the desired infinite-dimensional controller. This research fills the gap between the infinite-dimensional control design and finite-dimensional actuation in practice and suggests a promising direction for exploring PDE-based control design for soft robots.

==> bibtex.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{survey}
D.~Rus and M.~Tolley, ``Design, fabrication and control of soft robots,''
  \emph{Nature}, vol. 521, pp. 467--75, 05 2015.

\bibitem{PCC}
\BIBentryALTinterwordspacing
I.~Robert J.~Webster and B.~A. Jones, ``Design and kinematic modeling of
  constant curvature continuum robots: A review,'' \emph{The International
  Journal of Robotics Research}, vol.~29, no.~13, pp. 1661--1683, 2010.
  [Online]. Available: \url{https://doi.org/10.1177/0278364910368147}
\BIBentrySTDinterwordspacing

\bibitem{janabi2021cosserat}
F.~Janabi-Sharifi, A.~Jalali, and I.~D. Walker, ``Cosserat rod-based dynamic
  modeling of tendon-driven continuum robots: A tutorial,'' \emph{IEEE Access},
  vol.~9, pp. 68\,703--68\,719, 2021.

\bibitem{FEM_overview}
\BIBentryALTinterwordspacing
M.~S. Xavier, A.~J. Fleming, and Y.~K. Yong, ``Finite element modeling of soft
  fluidic actuators: Overview and recent developments,'' \emph{Advanced
  Intelligent Systems}, vol.~3, no.~2, p. 2000187, 2021. [Online]. Available:
  \url{https://onlinelibrary.wiley.com/doi/abs/10.1002/aisy.202000187}
\BIBentrySTDinterwordspacing

\bibitem{FEM}
C.~Duriez, ``Control of elastic soft robots based on real-time finite element
  method,'' in \emph{2013 IEEE International Conference on Robotics and
  Automation}, 2013, pp. 3982--3987.

\bibitem{issues_FEM}
\BIBentryALTinterwordspacing
O.~Goury and C.~Duriez, ``Fast, generic, and reliable control and simulation of
  soft robots using model order reduction,'' \emph{Trans. Rob.}, vol.~34,
  no.~6, p. 1565–1576, dec 2018. [Online]. Available:
  \url{https://doi.org/10.1109/TRO.2018.2861900}
\BIBentrySTDinterwordspacing

\bibitem{discrete}
C.~Della~Santina, C.~Duriez, and D.~Rus, ``Model based control of soft robots:
  A survey of the state of the art and open challenges,'' 10 2021.

\bibitem{simo1988dynamics}
J.~C. Simo and L.~Vu-Quoc, ``On the dynamics in space of rods undergoing large
  motions—a geometrically exact approach,'' \emph{Computer methods in applied
  mechanics and engineering}, vol.~66, no.~2, pp. 125--161, 1988.

\bibitem{Open_Loop}
\BIBentryALTinterwordspacing
J.~Wang and A.~Chortos, ``Control strategies for soft robot systems,''
  \emph{Advanced Intelligent Systems}, vol.~4, no.~5, p. 2100165, 2022.
  [Online]. Available:
  \url{https://onlinelibrary.wiley.com/doi/abs/10.1002/aisy.202100165}
\BIBentrySTDinterwordspacing

\bibitem{tongjia}
\BIBentryALTinterwordspacing
T.~Zheng and H.~Lin, ``Pde-based dynamic control and estimation of soft robotic
  arms,'' 2022. [Online]. Available: \url{https://arxiv.org/abs/2203.13724}
\BIBentrySTDinterwordspacing

\bibitem{rucker2011statics}
D.~C. Rucker and R.~J. Webster~III, ``Statics and dynamics of continuum robots
  with general tendon routing and external loading,'' \emph{IEEE Transactions
  on Robotics}, vol.~27, no.~6, pp. 1033--1044, 2011.

\bibitem{renda2014dynamic}
F.~Renda, M.~Giorelli, M.~Calisti, M.~Cianchetti, and C.~Laschi, ``Dynamic
  model of a multibending soft robot arm driven by cables,'' \emph{IEEE
  Transactions on Robotics}, vol.~30, no.~5, pp. 1109--1122, 2014.

\bibitem{zheng2022pde}
T.~Zheng and H.~Lin, ``Pde-based dynamic control and estimation of soft robotic
  arms,'' in \emph{2022 61st IEEE Conference on Decision and Control
  (CDC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022.

\bibitem{till2019real}
J.~Till, V.~Aloi, and C.~Rucker, ``Real-time dynamics of soft and continuum
  robots based on cosserat rod models,'' \emph{The International Journal of
  Robotics Research}, vol.~38, no.~6, pp. 723--746, 2019.

\bibitem{antman2005nonlinear}
S.~Antman, \emph{Nonlinear problems of elasticity}.\hskip 1em plus 0.5em minus
  0.4em\relax Springer Science \& Business Media, 2005, vol. 107.

\bibitem{FPAM}
N.~Naclerio and E.~Hawkes, ``Simple, low-hysteresis, foldable, fabric pneumatic
  artificial muscle,'' \emph{IEEE Robotics and Automation Letters}, vol.~PP,
  pp. 1--1, 02 2020.

\bibitem{SPAM}
\BIBentryALTinterwordspacing
J.~D. Greer, T.~K. Morimoto, A.~M. Okamura, and E.~W. Hawkes, ``Series
  pneumatic artificial muscles (spams) and application to a soft continuum
  robot,'' \emph{IEEE International Conference on Robotics and Automation :
  ICRA : [proceedings]. IEEE International Conference on Robotics and
  Automation}, vol. 2017, p. 5503—5510, 2017. [Online]. Available:
  \url{https://europepmc.org/articles/PMC5786173}
\BIBentrySTDinterwordspacing

\bibitem{pratt_1987}
\BIBentryALTinterwordspacing
V.~Pratt, ``Direct least-squares fitting of algebraic surfaces vaughan pratt,''
  Apr 1987. [Online]. Available: \url{http://boole.stanford.edu/pub/fit.pdf}
\BIBentrySTDinterwordspacing

\end{thebibliography}

